Selective Amnesia: On Efficient, High-Fidelity and Blind Suppression of Backdoor Effects in Trojaned Machine Learning Models

In this paper, we present a simple yet surprisingly effective technique to induce "selective amnesia" on a backdoored model. Our approach, called SEAM, has been inspired by the problem of catastrophic forgetting (CF), a long standing issue in continual learning. Our idea is to retrain a given DNN model on randomly labeled clean data, to induce a CF on the model, leading to a sudden forget on both primary and backdoor tasks; then we recover the primary task by retraining the randomized model on correctly labeled clean data. We analyzed SEAM by modeling the unlearning process as continual learning and further approximating a DNN using Neural Tangent Kernel for measuring CF. Our analysis shows that our random-labeling approach actually maximizes the CF on an unknown backdoor in the absence of triggered inputs, and also preserves some feature extraction in the network to enable a fast revival of the primary task. We further evaluated SEAM on both image processing and Natural Language Processing tasks, under both data contamination and training manipulation attacks, over thousands of models either trained on popular image datasets or provided by the TrojAI competition. Our experiments show that SEAM vastly outperforms the state-of-the-art unlearning techniques, achieving a high Fidelity (measuring the gap between the accuracy of the primary task and that of the backdoor) within a few minutes (about 30 times faster than training a model from scratch using the MNIST dataset), with only a small amount of clean data (0.1% of training data for TrojAI models).

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> backup.tex <==

\subsection{Neural Tangent Kernel (NTK)}

%\noindent\textbf{NTK}.
We followed the neural Tangent Kernel (NTK) theory for continual learning in our theoretical analyses. In a continual learning setup, we consider a sequence of tasks $\tau_{1}, \tau_{2}, \ldots, \tau_{T}, T \in \mathbb{N}^{*}$, in which each task is a supervised learning task with the input and output in the same high dimensional spaces, respectively. Consider the neural network was trained using the training data labeled for each of the $T$ tasks in a sequential order. [NTK][Doan] used NTK to measure the catastrophic forgetting (CF) of the task $\tau_{i-1}$ after the training of task $\tau_i$:

\begin{equation} \label{Taylor expansion}
    f_{\tau_i}^{*}(x)=f_{\tau_{i-1}}^{*}(x)+\left\langle\nabla_{\omega} f_{0}(x), \omega_{\tau_i}^{*}-\omega_{\tau_{i-1}}^{*}\right\rangle
\end{equation}

\noindent where $\omega^{\star}_{\tau_i}$ is the final weight after the training on task $\tau_i$, $\left\langle * \right\rangle$ represents the inner product in the kernel space. $\nabla_{\omega} f_{0}(x) = \phi(x)\ \in \mathbb{R}^{p}$ is defined as the NTK feature map for an input sample $x$, where $p$ is the number of weights in the neural networks and $f_0$ represents the initial state of the neural network before the first task $\tau_{1}$ is trained. Note that here the NTK is defined on the Taylor expansion around the initial state of the DNN ($f_0$), but it can be extended to the Taylor expansion around any state of the DNN in order to approximate a subsequent state of the DNN in the sequential training. Based on the definition of NTK (equation \ref{Taylor expansion}), we can prove the following corollary ~\ref{similarity} (see Appendex for the proof).

\begin{corollary}
\label{chain}
Any two tasks $\tau_S$ and $\tau_T$ that $\tau_S$ occurs before $\tau_T$ in the sequence of tasks satisfy.
\begin{equation} \label{task S to T}
f_{\tau_{T}}^{\star}(x) =f_{\tau_{S}}^{\star}(x)+\left\langle\phi(x), \omega_{\tau_{T}}^{\star}-\omega_{\tau_{S}}^{\star}\right\rangle
\end{equation}
\noindent where $\phi(x)\in \mathbb{R}^{p}$, is the NTK feature map. 
\end{corollary}

%\noindent\textbf{\OURMETHOD  under NTK}. 
\subsection{Measuring Catastrophic Forgetting (CF) using NTK}

\begin{definition}
Let $\tau_S$ and $\tau_T$ be the source and target tasks, respectively, where $\tau_S$ is trained before $\tau_T$ in a sequence of continual training tasks, and $D_{\tau_S}=(X_{\tau_S}, Y_{\tau_S})$ be the testing set of the source task. The CF of the model for the source task $f_{\tau_S}$ after the training of all the subsequent tasks until the target task $\tau_T$ is defined as:
\begin{equation}
    \begin{aligned}
\Delta^{\tau_{S} \rightarrow \tau_{T}}\left(X^{\tau_{S}}\right) &=\left\|\delta^{\tau_{S} \rightarrow \tau_{T}}\left(X^{\tau_{S}}\right)\right\|_{2}^{2} \\
&=\sum_{(x, y) \in \mathcal{D}_{\tau_{S}}}\left(f_{\tau_{T}}^{\star}(x)-f_{\tau_{S}}^{\star}(x)\right)^{2}
\end{aligned}
\end{equation}
\noindent where $f_{\tau_S}$ and $f_{\tau_T}$ represent the models for the source and target tasks, respectively.
\end{definition}

Note that $\delta^{\tau_{S} \rightarrow \tau_{T}}\left(X^{\tau_{S}}\right)$ is a vector in $\mathbb{R}^{n_{\tau_{S}}}$ ($n_{\tau_{S}}=|\mathcal{X}_{\tau_{S}}|$), in which each dimension represents the difference of the predicted output on an input sample $x$ (with the desirable output $y$) in $\mathcal{X}_{\tau_{S}}$ between the model for the source task $\tau_S$ and the model for in the target task $\tau_T$. In the case of multi-class classification, we represent the predicted output as an onehot vector in which $y_{k}=1$ for the predicted class $k$ and $y_{i}=0$ for all the other classes. %take the k-output of $f_{\tau}^{\star}$ such that $y_{k}=1$. 
To measure the CF on this task, we compute the squared
norm of the onehot vectors output by the models for the source and the target tasks, respectively.
Interestingly, the above expression of CF is general but has an interesting linear form under the NTK representation, which enable us to perform insightful analyses on the effectiveness of different forgetting approaches.

\begin{lemma}
\label{lemma_cf}
Let $\left\{\omega_{\tau}^{\star}, \forall \tau \in[T]\right\}$ be the weight at the end of the training of task $\tau$. The CF of a source task $\tau_S$ with respect to a target task $\tau_T$ is measured by:
\begin{equation} \label{lemma CF}
    \begin{aligned}
\Delta^{\tau_{S} \rightarrow \tau_{T}}\left(X^{\tau_{T}}\right) &=\left\|\delta^{\tau_{S} \rightarrow \tau_{T}}\left(X^{\tau_{T}}\right)\right\|_{2}^{2} \\
&=\left\|\phi\left(X^{\tau_{T}}\right)\left(\omega_{\tau_{T}}^{*}-\omega_{\tau_{S}}^{*}\right)\right\|_{2}^{2}
\end{aligned}
\end{equation}
See Appendix for the proof.
\end{lemma}

Further, as shown in ~\cite{bennani2020generalisation},

\begin{equation}\label{Bennani}
    \omega_{\tau_{T}}^{\star}-\omega_{\tau_{s}}^{\star}=\phi\left(X^{\tau_T}\right)^{\top}\left[\phi\left(X^{\tau_T}\right) \phi\left(X^{\tau_T}\right)^{\top}+\lambda I\right]^{-1} \tilde{y}_{\tau_T}
\end{equation}

\noindent where $\tilde{y}_{\tau_T} = {y}_{\tau_T} -f^{\star}_{\tau_s}(X^{\tau_T})$ is the {\em residual} between the desirable output and the predicted label by the source model on the training data of the target model $X^{\tau_T}$, $\lambda I$ is the regularization term for better lazy training to improve the precision of the Taylor expansion ~\cite{chizat2018lazy}.

Combining the equations \ref{lemma CF} and \ref{Bennani}, and applying the Single Value Decomposition (SVD) on the kernel matrix $\phi\left(X^{\tau_S}\right)$ ~\cite{doan2021theoretical}, we obtain the following corollary about the source and the target model.

\begin{corollary}
\blue {The CF of $\tau_S$'s training data $X^{\tau_S}$ from source task $\tau_S$ to the target task $\tau_T$ can be expressed as: }
\begin{equation}
%\scriptscriptstyle
\begingroup\makeatletter\def\f@size{5}\check@mathfonts
\def\maketag@@@#1{\hbox{\m@th\large\normalfont#1}}%
\begin{aligned}
\Delta^{\tau_S \rightarrow \tau_T}\left(X^{\tau_S}\right) &= \left\|
 \phi(X^{\tau_S}) \phi\left(X^{\tau_T}\right)^{\top}\left[\phi\left(X^{\tau_T}\right) \phi\left(X^{\tau_T}\right)^{\top}+\lambda I\right]^{-1} \tilde{y}_{\tau_T} \right\|_{2}^{2} \\&= \left\|
U_{{\tau_S}} \Sigma_{{\tau_S}} V_{{\tau_S}}^{\top} V_{\tau_T} \Sigma_{\tau_T}U_{\tau_T}^T\left[U_{\tau_T}\Sigma_{\tau_T}^{2}U_{\tau_T}^T+\lambda I\right]^{-1}  \tilde{y}_{\tau_T}\right\|_{2}^{2} \\&= \left\| U_{{\tau_S}} \Sigma_{{\tau_S}} \underbrace{V_{{\tau_S}}^{\top} V_{\tau_T}}_{O^{\tau_{S\rightarrow T}}} \Sigma_{\tau_T}\left[\Sigma_{\tau_T}^{2}+\lambda I\right]^{-1} U_{\tau_T}^{\top} \tilde{y}_{\tau_T}\right\|_{2}^{2}
\end{aligned}
%f_{\tau_S}^{\star}(x)=f_{\tau_T}^{\star}(x) + \phi(x) \phi\left(X^{\tau_S}\right)^{\top}\left[\phi\left(X^{\tau_S}\right) \phi\left(X^{\tau_S}\right)^{\top}+\lambda I\right]^{-1} \tilde{y}_{\tau_S}
\end{equation}
\end{corollary}

\noindent ~\cite{doan2021theoretical} showed that $O^{\tau_{S\rightarrow T}}=V_{\tau_{S}}^{\top} V_{\tau_T}$ is a good measure of the {\em similarity} between two tasks $\tau_S$ and $\tau_T$, which determines the CF of the source model (for the task $\tau_S$) on a specific input data $X_{\tau_S}$ after the training of the target task $\tau_T$. Intuitively, if the angle between the representation vectors in the models for these tasks on the same input samples (i.e., $X_{\tau_S}$) is small (i.e., these two tasks are similar), the update of the model weights by training for the target task $\tau_T$ will have high impact on a source task $\tau_{S}$.




\subsection{The Mechanism of Backdoor Forgetting}

Suppose a neural network $f_{\tau_P}^{*}$ was trained on the task $\tau_P$ using a poisoned dataset $D_p = \{X_p,Y_p\}$. The model may accomplish both the the primary classification task and the trigger recognition task, because $D_p$ may contain a subset of training samples containing a trigger, denoted as $D_t = \{X_t,Y_t\}$ where every $y_t \in Y_t$ represents the same class (i.e., the target class). 
The goal of the backdoor forgetting is to train a competitive task $\tau_F$ starting from the model $f_{\tau_P}^{*}$ using a dataset $D_{\tau_F}$ such that the backdoor (i.e., the trigger recognition task) is forgotten (i.e., unlearned) in the resulting model $f_{\tau_F}^{*}$. According to the NTK analyses described above, the CF from the model for the task $\tau_P$ to the competitive model for the task $\tau_F$ is:


\begin{equation} \label{P-F forget}
\begin{array}{ll}
&\Delta^{\tau_P \rightarrow \tau_F}(X ; X^{\tau_F}) = \\
&\left\| \phi(X) \phi\left(X^{\tau_F}\right)^{\top}\left[\phi\left(X^{\tau_F}\right)  \phi\left(X^{\tau_F}\right)^{\top}+\lambda I\right]^{-1} \tilde{y}_{\tau_F} \right\|_{2}^{2}
\end{array}
\end{equation}

\blue{Note that, in the RHS equ.\ref{P-F forget}, every terms after $\phi(x)$ are fixed once $\tau_P,\tau_F$ fixed. In another word, the variant $x$ is only exist in the first term $\phi(x)$.} Thus, we have the following theorem,

\begin{theorem} \label{forget thm}
\blue{When we have zero knowledge of trojan data, with only few clean data, and we hope to use this few data as a competitive task $\tau_F$ to maximize the CF $\Delta^{\tau_P \rightarrow \tau_F}\left(X_B\right)$. this CF can reach maximum when $\tilde{y}_{\tau_F}$ reach maximum, that is, 
if $||\tilde{y}_{\tau_F}||^2_2 \rightarrow + \infinity{\rotatebox{90}{8}}$, then $\Delta^{\tau_P \rightarrow \tau_F}(X_B) \rightarrow +\infinity{\rotatebox{90}{8}}$\\ }
\end{theorem}

%If we want to leverage $\tau_F$ to maximize this CF, which is to optimize the following equation:
%\begin{equation}
%    \argmax_{\tau_F}\Delta^{\tau_P \rightarrow \tau_F}\left(x\right)
%\end{equation}
%If $||\tilde{y}_{\tau_F}||^2_2 \rightarrow + \infinity{\rotatebox{90}{8}}$ then $\Delta^{\tau_P \rightarrow \tau_F} \rightarrow +\infinity{\rotatebox{90}{8}}$.

%The CF reach maximum when $\tilde{y}_{\tau_F}$ reach maximum. 
The proof of Theorem \ref{forget thm} is given in the Appendix. The theorem indicates that if we want to leverage a competitive task $\tau_F$ to maximize the CF of the task $\tau_P$, we should resort to the task that maximizes $\tilde{y}_{\tau_F}$, which can be achieved by using a dataset in which each sample has the desirable output (label) of ${y}_{\tau_S}$ that is different from their predicted output $f^{\star}_{\tau_T}(X^{\tau_S})$ by the source model.
Assuming we have small subset of training data $D_c = \{X_c,Y_c\}$, we may construct a dataset $D_{\tau_F}=\{X_c,Y_F\}$ by generating a random label for each sample $x \in X_c$ to replace $Y_c$.
According to Theorem \ref{forget thm}, this randomly labeled dataset  used in the SEAM approach for backdoor forgetting induces the maximum CF for any task learned by the model $f_{\tau_F}^{*}$, including any backdoor task as well as the primary classification task (note that the CF on the clean dataset $X_c$, $\Delta^{\tau_P \rightarrow \tau_F}\left(X_c\right)$ is also large).

%Observe Eq.\ref{P-F forget}, if we want To maximize the forgetting of trojan, the most significant part is the residual part. To maximize this residual term, we used uniform distribution to generate random labels to replace $Y_c$. So the $\tau_F$ becomes a random task. 
%ote after the training on the that after shuffle label, the new task $\tau_F$ do significant forget the trojan, but the clean data feature has also forgotten; if we let $x = X_c$ to measure forgetting of clean data, $\Delta^{\tau_P \rightarrow \tau_F}\left(X_c\right)$ is also large. That leads to the next step in the next section, to recover the clean data memory.

Equation \ref{P-F forget} also implies that the direct fine-tuning of the model $f_{\tau_P}^{*}$ using the clean dataset $D_C$ (equivalently, using the primary task as the competitive task) will not achieve effective forgetting of the backdoor, which is consistent with previous studies ~\cite{}.
%We first want to analysis that, when $||D_c||$ is small, using $D_c$ fine-tune $f_p$ cannot remove backdoor. in eq.\ref{P-F forget}. 
Replacing $x$ by the clean dataset $X_t$ in Equation \ref{P-F forget}, which is used in the fine-tuning, the residual term $\tilde{y}_{\tau_F} = {y}_{\tau_F} -f^{\star}_{\tau_P}(X^{\tau_F}) \approx 0$, because the model $f^{\star}_{\tau_P}$ is expected to predict most of the true class of the testing data of the primary task. \blue{Compare fine-tuning and competitive task $\tau_F$, in here they have the same  first term, $\phi(X_t) \phi(X^{\tau_F})^{\top}$, but the residual term for $\tau_F$ is significantly large, since the model $f^{\star}_{\tau_P}$ is  expected  to predict most of the different class of the testing data of the random task.} Intuitively, because the the initial model $f_{\tau_P}^{*}$ already makes correct prediction on most samples in the clean dataset $X_t$, fine-tuning does not change the model significantly, and thus the tasks in the model including the backdoor task will not be forgotten.

%\noindent\textbf{Theorem 1}. backdoor will be depressed.
%







%---------------------- old version ---------------------------
\ignore{

Plenty of research has shown that it is really easy to inject a trojan into DNN. The goal of attacker is that when the source class input contains Trojan, the output need to return the target class. Source agnostic trojan attack generalized this goal: No matter what input inference the target model with trigger, the trojan task goal let the target model always return target class. An example shows in fig.\ref{fig:traffic sign}. LHS is a regular training data, RHS is the LHS training data with a blue polygon trigger. Attacker use small propotion data like LHS and labeled as target class, so that model trained by this poisoned dataset will recognize this trigger, whenever a source class image with trigger input to the model, the prediction will then be the target class instead source class. 

\begin{figure}[htb]
    \centering % <-- added
\begin{subfigure}{0.1\textwidth}
  \includegraphics[width=\linewidth]{imgs/traffic_sign.png}
  \caption{Label = source class}
  \label{fig:1}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.1\textwidth}
  \includegraphics[width=\linewidth]{imgs/trojan_traffic_siggn.png}
  \caption{Label = target class}
  \label{fig:3}
\end{subfigure}

\caption{Data contaminates}
\label{fig:traffic sign}
\end{figure}
State of art DNN backdoor attacks are not only focused on data poisoning attack, some advanced attack like [Non-poisoning based attack] also shows great success to inject trojan. ~\cite{li2020backdoor} gives a comprehensive introduce of backdoor attack in DNN.


\subsection{Multi-task learning}
\blue{Multi-task learning is a concept of learning multiple task jointly, instead of learning them individually. It turns out that joint learning several related tasks can out-perform the training of each task individually~\cite{wang2020masking,zhou2019legal,zhao2021adjacency}. More specificly, in multi-task learning, we have several supervised learning tasks $\tau_t, t\in [T]$ where $\tau_t = \{x_{t_j},y_{t_j}\}^{n_t}_{j=1} }$, with $T\in \mathbb{N}^{\star}$. If $\mathcal{X}$ is a feature space of interest, and $\mathcal{X} = \mathbb{R}^p$, and $\mathcal{Y}$ is the space of labels ($\mathcal{Y} = \mathbb{R}$). While $X_{t} \in \mathbb{R}^{n_t \times p}$ ($p$ us the number of features) represents the dataset of task $\tau_t$ and $x_{i}^{t}, j=1, \ldots, n_{t} \in \mathcal{X}$ is a sample with its corresponding label $y_{i}^{t} \in \mathcal{Y}$. The goal of multi-task learning is to learn a function: $f_{\omega}:\mathcal{X} \times \mathcal{T} \rightarrow \mathcal{Y}$ with $\omega \in \mathbb{R}^{p}$ 
the parameters is going to fit the prediction as accurate as possible.}

\subsection{Neural tangent kernel} 
\blue{Neural network has always been considered as a black box model because the approximation given by the neural network will not offer much insight on the function $F$ it approximates. Recently, neural tangent kernel (NTK) provides a set of theoretical tools for understanding neural networks. In the NTK theory, a neural network is approximated by a kernel machine, in which the kernel function is composed of the gradient of neural network parameters with regard to the training data. %This brings a great help to the understanding of neural network mechanism and the theoretical understanding of neural network. 
More specifically, NTK used the Taylor expansion of the network function with respect to the weights around its initialization:
\begin{equation}\label{NTK_def}
    f(x, w) \approx f\left(x, w_{0}\right)+\nabla_{w} f\left(x, w_{0}\right)^{T}\left(w-w_{0}\right)
\end{equation}
\noindent where $w_{0}$ is neural network initial weights, $\nabla_{w} f\left(x, w_{0}\right)$ is referred to as the "NTK", which can be written in the form of a {\em feature map}:
\begin{equation}
    \phi(x)=\nabla_{w} f\left(x, w_{0}\right)
\end{equation}
where $\phi$ represent the feature map in the kernel (NTK) space. Note that, once we decide to perform the Taylor expansion around the initial weights $w_0$, the feature map $\phi$ is fixed, which means, even though the weight of the neural network will be updated during the training process, the representations of the input data are always approximated as feature vectors in the same kernel space. In practice, it is not necessary to perform the expansion around the initial weights $w_0$. In fact, the Taylor expansion can have better precision if the it is performed around the weights in a latter state $w_k,k>0$ when we aim to approximate the neural network after the state $k$. For more details of the NTK theory, We refer to the original paper ~\cite{}, and a recent implementation of the NTK framework for a convolutional neural network (CNN) ~\cite{}.}
\subsection{Threat model}

Defenders have the test set. 
}
